Threat Model-Agnostic Adversarial Defense using Diffusion Models

Deep Neural Networks (DNNs) are highly sensitive to imperceptible malicious perturbations, known as adversarial attacks. Following the discovery of this vulnerability in real-world imaging and vision applications, the associated safety concerns have attracted vast research attention, and many defense techniques have been developed. Most of these defense methods rely on adversarial training (AT) -- training the classification network on images perturbed according to a specific threat model, which defines the magnitude of the allowed modification. Although AT leads to promising results, training on a specific threat model fails to generalize to other types of perturbations. A different approach utilizes a preprocessing step to remove the adversarial perturbation from the attacked image. In this work, we follow the latter path and aim to develop a technique that leads to robust classifiers across various realizations of threat models. To this end, we harness the recent advances in stochastic generative modeling, and means to leverage these for sampling from conditional distributions. Our defense relies on an addition of Gaussian i.i.d noise to the attacked image, followed by a pretrained diffusion process -- an architecture that performs a stochastic iterative process over a denoising network, yielding a high perceptual quality denoised outcome. The obtained robustness with this stochastic preprocessing step is validated through extensive experiments on the CIFAR-10 dataset, showing that our method outperforms the leading defense methods under various threat models.

==> tables/full_yoon.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Robust accuracies on CIFAR-10 $L_{\infty}, \epsilon=8/255$ }
\label{table:cifar10-white-box}
\begin{tabular}{lcccccc}
\hline\noalign{\smallskip}
\hline
Defense & Attack & \multicolumn{2}{c}{Base Classifier} & \multicolumn{2}{c}{Preprocessed}\\
& & \multicolumn{2}{c}{Nat. Adv.} & \multicolumn{2}{c}{Nat. Adv.}\\
\hline\noalign{\smallskip}
~\cite{yoon2021adversarial} & grey-box & 95.60 & 00.00 & 86.39 & 80.49 \\
~\cite{yoon2021adversarial}* & grey-box & 95.60 & 00.00 & 86.39 & 80.49 \\
\hline\noalign{\smallskip}
~\cite{yoon2021adversarial} & BPDA+EOT & 95.60 & 00.00 & 86.39 & 69.03 \\
~\cite{yoon2021adversarial}* & BPDA+EOT & 95.60 & 00.00 & 86.39 & 44.79 \\
\hline\noalign{\smallskip}
~\cite{yoon2021adversarial} & white-box &  95.60 & 00.00 & 86.39 & 60.77 \\
~\cite{yoon2021adversarial}* & white-box & 95.60 & 00.00 & 86.39 & 31.42 \\
\hline\noalign{\smallskip}


\hline
\end{tabular}
\end{center}
\end{table}

